GNU Aris: a web application for students

We report on recent improvements to the free logic education software tool GNU Aris, including the latest features added during the Google Summer of Code 2023 project. We focused on making GNU Aris a web application to enable almost all users to use it as a standalone offline web application written in a combination of HTML, JavaScript, and WebAssembly. We used the Qt Quick framework with Emscripten to compile the application to WebAssembly. In the report we summarize the user feedback of university students given during a course on logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{42}
\providecommand{\publicationstatus}{J. Narboux, W. Neuper and P. Quaresma (Eds.): Theorem Proving\\ Components for Educational Software 2024 (ThEdu'24)\\
EPTCS 419, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.419.3}{10.4204/EPTCS.419.3}}
\pdfoutput=1

